NFT Bubbles

By investigating nonfungible tokens (NFTs), we provide the first systematic study of retail investor behavior through asset bubbles. Given that NFTs are recorded in public blockchains, we are able to track investor behavior over time, leading to the identification of numerous price run-ups and crashes. Our study reveals that agent-level variables, such as investor sophistication, heterogeneity, and wash trading, in addition to aggregate variables, such as volatility, price acceleration, and turnover, significantly predict bubble formation and price crashes. We find that sophisticated investors consistently outperform others and exhibit characteristics consistent with superior information and skills, supporting the narrative surrounding asset pricing bubbles.

==> Arxiv March 2023/TAB/fama_reg.tex <==
\begin{tabular}{lccccc}
\toprule
              & (1)     & (2)      & (3)     & (4)     & (5)      \\
Dep. Variable & $\;\quad\,$Crash$\;\quad\,$     & $\;\quad\,$Crash$\;\quad\,$      & $\;\quad\,$Crash$\;\quad\,$     & $\;\quad\,$Crash$\;\quad\,$     & $\;\quad\,$Crash$\;\quad\,$      \\
\midrule
              &           &            &           &           &            \\
Volatility    & 0.4401*** &            &           &           & 0.2714***   \\
              & (7.2525)  &            &           &           & (4.5709)    \\[1.0em]
Turnover      &           & -0.3768*** &           &           & -0.3199***  \\
              &           & (-5.5371)  &           &           & (-5.5626)   \\[1.0em]
Age           &           &            & 0.0001*** &           & 0.0001***   \\
              &           &            & (4.0524)  &           & (3.1493)    \\[1.0em]
Acceleration  &           &            &           & 0.1668*** & 0.1594***   \\
              &           &            &           & (11.344)  & (10.557)    \\[1.0em]
Intercept     & 0.2582*** & 0.5431***  & 0.4751*** & 0.3335*** & 0.1669***   \\
              & (6.6416)  & (30.182)   & (24.898)  & (15.626)  & (3.9723)    \\[0.1em]
              &           &            &           &           &            \\
Observations & 1,017 & 1,017 & 1,017 & 1,017 & 1,017 \\
R-squared             & 0.0468 & 0.0192 & 0.0217 & 0.1601 & 0.2110 \\
\bottomrule
\end{tabular}

==> Arxiv March 2023/TAB/fama_reg_agent.tex <==
\begin{tabular}{lcccccc}
\toprule
              &   (1)      &   (2)      &   (3)      &   (4)          &   (5)          &   (6)         \\
Dep. Variable & Crash        & Crash          & Crash        & Ex-Post Return     & Ex-Post Return     & Ex-Post Return \\
\midrule
  &  &  &  &  &  &  \\
Sophisticated & -0.5114***   &                & -0.4155***   & 2.1993***    &              & 1.7250***   \\
              & (-3.4262)    &                & (-2.8422)    & (4.8323)     &              & (3.8923)    \\[1.0em]
Unique Owners & -0.0114*     &                & -0.0070      & 0.0585***    &              & 0.0403**    \\
              & (-1.8545)    &                & (-1.0926)    & (3.1115)     &              & (1.9849)    \\[1.0em]
Wash Trading  & 0.0770***    &                & 0.0613***    & -0.2718***   &              & -0.1988***  \\
              & (6.6193)     &                & (5.0739)     & (-7.7302)    &              & (-6.4099)   \\[1.0em]
Volatility    &              & 0.2714***      & 0.1785***    &              & -1.3846***   & -1.0269***  \\
              &              & (4.5709)       & (2.9338)     &              & (-9.0643)    & (-5.9488)   \\[1.0em]
Turnover      &              & -0.3199***     & -0.2224***   &              & 1.0092***    & 0.6125**    \\
              &              & (-5.5626)      & (-3.9693)    &              & (4.8642)     & (2.1825)    \\[1.0em]
Age           &              & 0.0001***      & 0.0001       &              & -0.0002***   & -0.0002     \\
              &              & (3.1493)       & (0.0698)     &              & (-4.9529)    & (-0.3302)   \\[1.0em]
Acceleration  &              & 0.1594***      & 0.1613***    &              & -0.5686***   & -0.5767***  \\
              &              & (10.557)       & (10.781)     &              & (-12.267)    & (-12.848)   \\[1.0em]
Intercept     & 0.5183***    & 0.1669***      & 0.2400***    & -0.6695***   & 0.9322***    & 0.5826***   \\
              & (15.389)     & (3.9723)       & (4.8339)     & (-7.1665)    & (8.5946)     & (4.0961)    \\[0.1em]
&  &  &  &  &  &  \\
Observations & 1,017 & 1,017 & 1,017 & 1,017 & 1,017 & 1,017 \\[0.1em]
R-squared             & 0.0700 & 0.2110 & 0.2391 & 0.1263 & 0.3641 & 0.4101 \\[0.25em]
\bottomrule
\end{tabular}

==> Arxiv March 2023/TAB/other_agents.tex <==
\begin{tabular}{lrrrrrr}
 & Count & Mean & Std & 10\% & 50\% & 90\% \\
Absolute Profits & 543,086 & 0.26 & 1.72 & -0.14 & 0.07 & 0.79 \\
Percentage Profits & 543,086 & 72.33 & 164.20 & -25.97 & 29.31 & 193.52 \\
Volume (ETH) & 543,086 & 0.93 & 2.53 & 0.09 & 0.33 & 1.83 \\
Volume (USD) & 543,086 & 2,054.49 & 5,573.14 & 186.61 & 712.51 & 3,984.74 \\
Holding Period (hours) & 543,086 & 4.86 & 8.09 & 0.00 & 0.42 & 17.54 \\
Trades & 543,086 & 1.84 & 2.56 & 1.00 & 1.00 & 3.00 \\
\end{tabular}


==> Arxiv March 2023/TAB/other_agents_2.tex <==
\begin{tabular}{lrrrrrr}
 & Count & Mean & Std & 10\% & 50\% & 90\% \\
Absolute Profits & 254,636 & 0.30 & 2.57 & -0.17 & 0.10 & 0.98 \\
Percentage Profits & 254,636 & 69.31 & 147.56 & -21.78 & 30.74 & 183.78 \\
Volume (ETH) & 254,636 & 1.42 & 4.36 & 0.10 & 0.47 & 2.77 \\
Volume (USD) & 254,636 & 3,097.47 & 9,593.96 & 219.20 & 1,010.02 & 5,994.40 \\
Holding Period (hours) & 254,636 & 5.73 & 8.26 & 0.00 & 1.36 & 18.37 \\
Trades & 254,636 & 3.00 & 5.12 & 1.00 & 2.00 & 6.00 \\
\end{tabular}


==> Arxiv March 2023/TAB/other_agents_diff.tex <==
\begin{tabular}{lrrrl}
 & Sophisticated & Others & Difference & t-stat \\
NFT Percentage Profits & 94.92 & 69.41 & 25.51 & 44.59*** \\
NFT Volume (ETH) & 8.49 & 1.43 & 7.06 & 98.37*** \\
NFT Holding Period (hours) & 7.76 & 5.72 & 2.04 & 62.25*** \\
NFT Trades & 22.41 & 3.05 & 19.36 & 136.26*** \\
Transactions & 1,088.48 & 273.17 & 815.30 & 123.40*** \\
Transacted Value & 631.61 & 220.70 & 410.91 & 13.83*** \\
Age (days) & 519.13 & 429.89 & 89.24 & 50.24*** \\
DEX Swaps & 75.24 & 24.40 & 50.83 & 34.59*** \\
DEX Liquidity & 3.58 & 1.25 & 2.32 & 19.64*** \\
DeFi Lending & 0.30 & 0.08 & 0.22 & 6.17*** \\
DeFi Borrowing & 0.79 & 0.27 & 0.52 & 6.99*** \\
\end{tabular}


==> Arxiv March 2023/TAB/reg_agent_based.tex <==
\begin{tabular}{lcccccc}
\toprule
Dep. Variable & Crash      & Crash      & Crash      & Ex-Post Return & Ex-Post Return & Ex-Post Return \\
\midrule
              &            &            &            &               &                &               \\
Sophisticated & -0.5473*** &            & -0.3756**  & 1.7142***     &                & 1.3000***     \\
              & (-3.4438)  &            & (-2.3915)  & (5.4086)      &                & (3.9364)      \\[1.0em]
Unique Owners & -0.0044*** &            & -0.0024*   & 0.0046        &                & 0.0001        \\
              & (-2.9865)  &            & (-1.8979)  & (1.1862)      &                & (0.0410)      \\[1.0em]
volatility    &            & 0.2643***  & 0.2320***  &               & -0.5897***     & -0.4978***    \\
              &            & (4.4068)   & (3.8361)   &               & (-5.1156)      & (-4.0387)     \\[1.0em]
turnover      &            & -0.3225*** & -0.2892*** &               & 0.7562***      & 0.6943***     \\
              &            & (-5.6004)  & (-5.3015)  &               & (4.3442)       & (3.7041)      \\[1.0em]
age           &            & 0.0001***  & 0.0001***  &               & -0.0002***     & -0.0002***    \\
              &            & (3.1030)   & (2.9891)   &               & (-5.8990)      & (-5.6074)     \\[1.0em]
acceleration  &            & 0.1629***  & 0.1635***  &               & -0.1712***     & -0.1739***    \\
              &            & (10.515)   & (10.268)   &               & (-6.8268)      & (-6.7466)     \\[1.0em]
Intercept     & 0.6193***  & 0.1704***  & 0.2514***  & -0.5091***    & 0.3686***      & 0.1093        \\
              & (19.578)    & (3.9879)  & (5.0638)   & (-9.8511)     & (4.3647)       & (0.9980)      \\
              &            &            &            &               &                &               \\
Observations  & 992        & 992        & 992        & 992           & 992            & 992           \\
R-squared     & 0.0194     & 0.2170     & 0.2244     & 0.0338        & 0.1380         & 0.1548        \\[1.0em]
\bottomrule
\end{tabular}

==> Arxiv March 2023/TAB/reg_ex_post_liquidity.tex <==
\begin{tabular}{lccccccccc}
\toprule
 & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) \\
Dep. Variable         & Turnover & Amihud & Volatility & Turnover & Amihud & Volatility & Turnover & Amihud & Volatility\\
\midrule
  &  &  &  &  &  &  &  &  &  \\
Crash Dummy   & -0.03***        & 0.0***        & 0.11***         &                 &               &                   &                 &               &              \\
              & (-6.04)         & (3.23)        & (7.09)          &                 &               &                   &                 &               &              \\[1.0em]
Unique Owners &                 &               &                   & 0.01***         & -0.0***       & -0.02***          &                 &               &            \\
              &                 &               &                   & (5.58)          & (-4.93)       & (-6.43)         &                 &               &              \\[1.0em]
Wash Trading  &                 &               &                   &                 &               &                   & -0.01***      & 0.01        & 0.02***         \\
              &                 &               &                   &                 &               &                   & (-8.63)       & (1.18)      & (2.85)         \\[1.0em]
Intercept     & 0.04***         & 0.01***       & 0.48***           & 0.02***         & 0.01***       & 0.56***           & 0.04***         & 0.01***       & 0.51***    \\
              & (9.53)          & (5.10)        & (35.57)           & (8.51)          & (12.14)       & (50.46)           & (10.89)         & (8.25)        & (40.57)    \\
&  &  &  &  &  &  &  &  &  \\
Observations & 1,017 & 1,017 & 1,017 & 1,017 & 1,017 & 1,017 & 1,017 & 1,017 & 1,017 \\[0.1em]
R-squared             & 0.04 & 0.01 & 0.05 & 0.12 & 0.01 & 0.04 & 0.06 & 0.00 & 0.01 \\[0.25em]
\bottomrule
\end{tabular}

==> Arxiv March 2023/TAB/reg_sophi.tex <==
\begin{tabular}{lcccccc}
 & (1) & (2) & (3) & (4) & (5) & (6) \\
Dep. Variable         & Future Return & Crash Dummy & Future Return & Future Return & Crash Dummy & Crash Dummy \\
  &  &  &  &  &  &  \\
Sophisticated & 2.5921***              & -0.5843***   &                        & 1.7407***              &                & -0.3895**      \\
                      & (5.5219)               & (-3.6838)    &                        & (3.6893)               &                & (-2.4805)      \\
volatility            &                        &              & -1.3616***             & -1.2391***             & 0.2643***      & 0.2369***      \\
                      &                        &              & (-9.0427)              & (-7.7859)              & (4.4068)       & (3.9267)       \\
turnover              &                        &              & 1.0200***              & 0.9383***              & -0.3225***     & -0.3042***     \\
                      &                        &              & (4.9195)               & (4.3187)               & (-5.6004)      & (-5.4675)      \\
age                   &                        &              & -0.0002***             & -0.0002***             & 5.664e-05***   & 5.614e-05***   \\
                      &                        &              & (-4.8043)              & (-4.5439)              & (3.1030)       & (3.0350)       \\
acceleration          &                        &              & -0.5780***             & -0.5815***             & 0.1629***      & 0.1637***      \\
                      &                        &              & (-12.196)              & (-11.837)              & (10.515)       & (10.247)       \\
Intercept & -1.0327***             & 0.6202***    & 0.9134***              & 0.5667***              & 0.1704***      & 0.2480***      \\
                      & (-12.484)              & (19.571)     & (8.4296)               & (4.1454)               & (3.9879)       & (5.0004)       \\
  &  &  &  &  &  &  \\
Observations & 992 & 992 & 992 & 992 & 992 & 992 \\
R-squared             & 0.0317 & 0.0132 & 0.3743 & 0.3879 & 0.2170 & 0.2226 \\
\end{tabular}


==> Arxiv March 2023/TAB/reg_sophi_description.tex <==
\begin{tabular}{lcccc}
 & (1) & (2) & (3) & (4) \\
Dep. Variable           & Absolute Profits     & Percentage Profits     & Volume (ETH)     & Holding Period (hours)     \\
  &  &  &  &  \\
Sophisticated & 0.0214***            & 15.945***              & -0.0272***       & -1.1330***                 \\
                        & (7.8519)             & (4.7400)               & (-8.4040)        & (-13.558)                  \\
Intercept & 0.1131***            &                        &                  &                            \\
                        & (144.11)             &                        &                  &                            \\
  &  &  &  &  \\
Observations & 738,419 & 738,419 & 738,419 & 738,419 \\
R-squared               & 0.2977 & 0.2267 & 0.6521 & 0.1269 \\
Time FEs &  &  &  &  \\
Event FEs & Yes & Yes & Yes & Yes \\
\end{tabular}


==> Arxiv March 2023/TAB/reg_sophi_description_2.tex <==
\begin{tabular}{lcccccccccc}
 & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) \\
Dep. Variable         & Percentage Profits   & Volume (ETH)   & Holding Period (hours)   & Trades      & Transactions & Total Value & Inception & DEX Liquidity & liquid      & Sophisticated \\
  &  &  &  &  &  &  &  &  &  &  \\
Sophisticated & 22.177***            & 6.6398***      & 1.8220***                & 18.693***   & 715.74***      & 274.28***   & -15.478***     & 35.819***   & 1.4487***   & 1.0000***       \\
                      & (34.028)             & (91.268)       & (49.537)                 & (130.90)    & (106.01)       & (24.137)    & (-8.1788)      & (28.347)    & (17.034)    & (3.967e+16)     \\
Intercept & 72.745***            & 1.8545***      & 5.9422***                & 3.7157***   & 372.74***      & 273.25***   & 1.876e+04***   & 36.405***   & 1.8551***   & -1.274e-15***   \\
                      & (169.20)             & (125.18)       & (252.68)                 & (208.54)    & (218.53)       & (60.970)    & (2.111e+04)    & (89.628)    & (62.793)    & (-352.29)       \\
  &  &  &  &  &  &  &  &  &  &  \\
Observations & 159,037 & 159,037 & 159,037 & 159,037 & 159,037 & 159,037 & 159,037 & 159,037 & 159,037 & 159,037 \\
R-squared             & 0.0043 & 0.1116 & 0.0094 & 0.2448 & 0.1260 & 0.0046 & 0.0004 & 0.0081 & 0.0027 & 1.0000 \\
\end{tabular}


==> Arxiv March 2023/TAB/reg_timing.tex <==
\begin{tabular}{lcccccc}
\toprule
 & (1) & (2) & (3) & (4) & (5) & (6) \\
Dep. Variable         & Timing & Buy Timing & Sell Timing & Timing & Buy Timing & Sell Timing \\
\midrule
  &  &  &  &  &  &  \\
Sophisticated (time-varying)  & 0.0209***    & 0.0100***        & 0.0107***        &              &                  &                  \\
                              & (12.791)     & (6.0698)         & (14.365)         &              &                  &                  \\[1.0em]
Sophisticated (constant)      &              &                  &                  & 0.0204***    & 0.0080***        & 0.0118***        \\
                              &              &                  &                  & (16.356)     & (6.3915)         & (22.123)         \\[1.0em]
Intercept                     & 0.4971***    & 0.4992***        & 0.4991***        & 0.4930***    & 0.4979***        & 0.4965***        \\
                              & (839.90)     & (846.56)         & (2077.1)         & (766.76)     & (778.76)         & (1998.2)         \\[1.0em]
  &  &  &  &  &  &  \\
Observations & 214,855 & 214,855 & 214,855 & 214,855 & 214,855 & 214,855 \\
R-squared             & 0.0011 & 0.0003 & 0.0015 & 0.0016 & 0.0003 & 0.0028 \\
\bottomrule
\end{tabular}


==> Arxiv March 2023/TAB/sophi_agents.tex <==
\begin{tabular}{lrrrrrr}
 & Count & Mean & Std & 10\% & 50\% & 90\% \\
Absolute Profits & 144,121 & 0.39 & 1.89 & -0.12 & 0.10 & 1.00 \\
Percentage Profits & 144,121 & 81.07 & 174.20 & -22.25 & 34.77 & 206.25 \\
Volume (ETH) & 144,121 & 1.00 & 2.53 & 0.10 & 0.38 & 2.00 \\
Volume (USD) & 144,121 & 2,184.85 & 5,646.06 & 193.38 & 784.60 & 4,423.79 \\
Holding Period (hours) & 144,121 & 4.56 & 7.44 & 0.00 & 0.80 & 15.82 \\
Trades & 144,121 & 2.37 & 3.50 & 1.00 & 1.00 & 4.00 \\
\end{tabular}


==> Arxiv March 2023/TAB/sophi_agents_2.tex <==
\begin{tabular}{lrrrrrr}
 & Count & Mean & Std & 10\% & 50\% & 90\% \\
Absolute Profits & 35,453 & 3.66 & 8.41 & 0.20 & 1.50 & 8.17 \\
Percentage Profits & 35,453 & 95.01 & 91.55 & 24.61 & 70.22 & 189.00 \\
Volume (ETH) & 35,453 & 8.45 & 13.29 & 1.18 & 3.99 & 19.22 \\
Volume (USD) & 35,453 & 18,776.99 & 29,943.63 & 2,459.16 & 8,682.58 & 43,264.85 \\
Holding Period (hours) & 35,453 & 7.76 & 5.28 & 1.86 & 6.90 & 14.60 \\
Trades & 35,453 & 22.35 & 26.47 & 6.00 & 13.00 & 47.00 \\
\end{tabular}


==> Arxiv March 2023/TAB/sophi_diff.tex <==
\begin{tabular}{lrrrr}
\toprule
                           & Sophisticated & Others & Difference & t-stat    \\
\midrule
%
\color{electric_blue}{\textbf{NFT Market}}\color{black} \\
Number of Trades           $\qquad\qquad$& 22.41         & 3.05   & 19.36      & 136.26*** \\
Traded Volume (ETH)        $\qquad\qquad$& 8.49          & 1.43   & 7.06       & 98.37***  \\
Percentage Profits         $\qquad\qquad$& 94.92         & 69.41  & 25.51      & 44.59***  \\
Holding Period (hours)     $\qquad\qquad$& 7.76          & 5.72   & 2.04       & 62.25***  \\[1em]

%
\color{electric_blue}\textbf{Blockchain}\color{black} \\
Number of Transactions     $\qquad\qquad$& 1,088.48      & 273.17 & 815.30     & 123.40*** \\
Transacted Value           $\qquad\qquad$& 631.61        & 220.70 & 410.91     & 13.83***  \\
Age (days)                 $\qquad\qquad$& 519.13        & 429.89 & 89.24      & 50.24***  \\
DEX Swaps                  $\qquad\qquad$& 75.24         & 24.40  & 50.83      & 34.59***  \\
DEX Liquidity              $\qquad\qquad$& 3.58          & 1.25   & 2.32       & 19.64***  \\
DeFi Lending               $\qquad\qquad$& 0.30          & 0.08   & 0.22       & 6.17***   \\
DeFi Borrowing             $\qquad\qquad$& 0.79          & 0.27   & 0.52       & 6.99***   \\
\bottomrule
\end{tabular}

==> Arxiv March 2023/TAB/summary_panel.tex <==
\begin{tabular}{lrrrrrr}
 & count & mean & std & 10\% & 50\% & 90\% \\
Price & 3,511,676 & 0.92 & 2.19 & 0.04 & 0.22 & 2.01 \\
Floor & 3,534,040 & 0.80 & 2.05 & 0.03 & 0.18 & 1.73 \\
Return & 3,508,406 & 5.63 & 44.04 & -16.46 & 0.00 & 19.62 \\
Volume & 3,535,662 & 1.24 & 4.42 & 0.00 & 0.00 & 2.38 \\
Sales & 3,535,662 & 1.66 & 4.42 & 0.00 & 0.00 & 4.00 \\
Minted & 3,535,662 & 8,102.61 & 7,998.05 & 623.00 & 7,795.00 & 11,312.00 \\
Supply & 3,440,668 & 6,467.23 & 9,027.44 & 341.00 & 3,974.00 & 11,111.00 \\
Turnover & 3,439,122 & 0.33 & 1.34 & 0.00 & 0.02 & 0.46 \\
Capitalization & 3,534,040 & 5,254.65 & 15,264.94 & 70.83 & 1,100.31 & 9,745.52 \\
Age & 3,535,662 & 2,739.42 & 2,095.13 & 443.00 & 2,307.00 & 5,648.00 \\
\end{tabular}


==> Arxiv March 2023/TAB/summary_stats.tex <==
\begin{tabular}{lrrrrrr}
\toprule
                   &$\quad$ Count  $\quad$   &$\quad$ Mean  $\quad$   &$\quad$ Std  $\quad$     &$\quad$ 10\%$\quad$   &$\quad$ 50\%$\quad$     &$\quad$ 90\%$\quad$      \\
\midrule
\textit{Price} ($\Xi$)      & 3,511,676 & 0.92     & 2.19      & 0.04   & 0.22     & 2.01      \\
\textit{Floor} ($\Xi$)      & 3,534,040 & 0.80     & 2.05      & 0.03   & 0.18     & 1.73      \\
\textit{Return} (\%)        & 3,508,406 & 5.63     & 44.04     & -16.46 & 0.00     & 19.62     \\
\textit{Volume} ($\Xi$)     & 3,535,662 & 1.24     & 4.42      & 0.00   & 0.00     & 2.38      \\
\textit{Sales}              & 3,535,662 & 1.66     & 4.42      & 0.00   & 0.00     & 4.00      \\
\textit{Minted}             & 3,535,662 & 8,102.61 & 7,998.05  & 623.00 & 7,795.00 & 11,312.00 \\
\textit{Supply}             & 3,440,668 & 6,467.23 & 9,027.44  & 341.00 & 3,974.00 & 11,111.00 \\
\textit{Turnover} (\%)      & 3,439,122 & 0.33     & 1.34      & 0.00   & 0.02     & 0.46      \\
\textit{Market Cap} ($\Xi$) & 3,534,040 & 5,254.65 & 15,264.94 & 70.83  & 1,100.31 & 9,745.52  \\
\textit{Age (hours)}        & 3,535,662 & 2,739.42 & 2,095.13  & 443.00 & 2,307.00 & 5,648.00  \\
\bottomrule
\end{tabular}

==> Arxiv March 2023/TAB/wash_exchanges.tex <==
\begin{tabular}{lrrrrrrr}
%\toprule
            & Total Volume        & Wash Volume         & Wash \% &  & Total Trades & Wash Trades & Wash \% \\
\midrule
OpenSea     & 32,797,993,136 \$ & 761,535,142 \$    & 2.32\%         &  & 27,270,308   & 181,410     & 0.67\%         \\
LooksRare   & 26,590,247,528 \$ & 26,064,869,084 \$ & 98.02\%        &  & 115,288      & 27,247      & 23.63\%        \\
X2Y2        & 4,025,756,413 \$  & 3,432,460,213 \$  & 85.26\%        &  & 587,407      & 125,241     & 21.32\%        \\
CryptoPunks & 2,495,977,352 \$  & 28,220,202 \$     & 1.13\%         &  & 22,427       & 328         & 1.46\%         \\
Blur        & 1,311,868,278 \$  & 142,010,668 \$    & 10.83\%        &  & 1,766,529    & 27,044      & 1.53\%         \\
\bottomrule
\end{tabular}

==> TAB/other_agents.tex <==
\begin{tabular}{lrrrrrr}
 & Count & Mean & Std & 10\% & 50\% & 90\% \\
Absolute Profits & 543,086 & 0.26 & 1.72 & -0.14 & 0.07 & 0.79 \\
Percentage Profits & 543,086 & 72.33 & 164.20 & -25.97 & 29.31 & 193.52 \\
Volume (ETH) & 543,086 & 0.93 & 2.53 & 0.09 & 0.33 & 1.83 \\
Volume (USD) & 543,086 & 2,054.49 & 5,573.14 & 186.61 & 712.51 & 3,984.74 \\
Holding Period (hours) & 543,086 & 4.86 & 8.09 & 0.00 & 0.42 & 17.54 \\
Trades & 543,086 & 1.84 & 2.56 & 1.00 & 1.00 & 3.00 \\
\end{tabular}


==> TAB/other_agents_2.tex <==
\begin{tabular}{lrrrrrr}
 & Count & Mean & Std & 10\% & 50\% & 90\% \\
Absolute Profits & 254,636 & 0.30 & 2.57 & -0.17 & 0.10 & 0.98 \\
Percentage Profits & 254,636 & 69.31 & 147.56 & -21.78 & 30.74 & 183.78 \\
Volume (ETH) & 254,636 & 1.42 & 4.36 & 0.10 & 0.47 & 2.77 \\
Volume (USD) & 254,636 & 3,097.47 & 9,593.96 & 219.20 & 1,010.02 & 5,994.40 \\
Holding Period (hours) & 254,636 & 5.73 & 8.26 & 0.00 & 1.36 & 18.37 \\
Trades & 254,636 & 3.00 & 5.12 & 1.00 & 2.00 & 6.00 \\
\end{tabular}


==> TAB/other_agents_diff.tex <==
\begin{tabular}{lrrrl}
 & Sophisticated & Others & Difference & t-stat \\
NFT Percentage Profits & 94.92 & 69.41 & 25.51 & 44.59*** \\
NFT Volume (ETH) & 8.49 & 1.43 & 7.06 & 98.37*** \\
NFT Holding Period (hours) & 7.76 & 5.72 & 2.04 & 62.25*** \\
NFT Trades & 22.41 & 3.05 & 19.36 & 136.26*** \\
Transactions & 1,088.48 & 273.17 & 815.30 & 123.40*** \\
Transacted Value & 631.61 & 220.70 & 410.91 & 13.83*** \\
Age (days) & 519.13 & 429.89 & 89.24 & 50.24*** \\
DEX Swaps & 75.24 & 24.40 & 50.83 & 34.59*** \\
DEX Liquidity & 3.58 & 1.25 & 2.32 & 19.64*** \\
DeFi Lending & 0.30 & 0.08 & 0.22 & 6.17*** \\
DeFi Borrowing & 0.79 & 0.27 & 0.52 & 6.99*** \\
\end{tabular}


==> TAB/reg_agent_based.tex <==
\begin{tabular}{lcccccc}
\toprule
Dep. Variable & Crash      & Crash      & Crash      & Ex-Post Return & Ex-Post Return & Ex-Post Return \\
\midrule
              &            &            &            &               &                &               \\
Sophisticated & -0.5473*** &            & -0.3756**  & 1.7142***     &                & 1.3000***     \\
              & (-3.4438)  &            & (-2.3915)  & (5.4086)      &                & (3.9364)      \\[1.0em]
Unique Owners & -0.0044*** &            & -0.0024*   & 0.0046        &                & 0.0001        \\
              & (-2.9865)  &            & (-1.8979)  & (1.1862)      &                & (0.0410)      \\[1.0em]
volatility    &            & 0.2643***  & 0.2320***  &               & -0.5897***     & -0.4978***    \\
              &            & (4.4068)   & (3.8361)   &               & (-5.1156)      & (-4.0387)     \\[1.0em]
turnover      &            & -0.3225*** & -0.2892*** &               & 0.7562***      & 0.6943***     \\
              &            & (-5.6004)  & (-5.3015)  &               & (4.3442)       & (3.7041)      \\[1.0em]
age           &            & 0.0001***  & 0.0001***  &               & -0.0002***     & -0.0002***    \\
              &            & (3.1030)   & (2.9891)   &               & (-5.8990)      & (-5.6074)     \\[1.0em]
acceleration  &            & 0.1629***  & 0.1635***  &               & -0.1712***     & -0.1739***    \\
              &            & (10.515)   & (10.268)   &               & (-6.8268)      & (-6.7466)     \\[1.0em]
Intercept     & 0.6193***  & 0.1704***  & 0.2514***  & -0.5091***    & 0.3686***      & 0.1093        \\
              & (19.578)    & (3.9879)  & (5.0638)   & (-9.8511)     & (4.3647)       & (0.9980)      \\
              &            &            &            &               &                &               \\
Observations  & 992        & 992        & 992        & 992           & 992            & 992           \\
R-squared     & 0.0194     & 0.2170     & 0.2244     & 0.0338        & 0.1380         & 0.1548        \\[1.0em]
\bottomrule
\end{tabular}

==> TAB/reg_sophi.tex <==
\begin{tabular}{lcccccc}
 & (1) & (2) & (3) & (4) & (5) & (6) \\
Dep. Variable         & Future Return & Crash Dummy & Future Return & Future Return & Crash Dummy & Crash Dummy \\
  &  &  &  &  &  &  \\
Sophisticated & 2.5921***              & -0.5843***   &                        & 1.7407***              &                & -0.3895**      \\
                      & (5.5219)               & (-3.6838)    &                        & (3.6893)               &                & (-2.4805)      \\
volatility            &                        &              & -1.3616***             & -1.2391***             & 0.2643***      & 0.2369***      \\
                      &                        &              & (-9.0427)              & (-7.7859)              & (4.4068)       & (3.9267)       \\
turnover              &                        &              & 1.0200***              & 0.9383***              & -0.3225***     & -0.3042***     \\
                      &                        &              & (4.9195)               & (4.3187)               & (-5.6004)      & (-5.4675)      \\
age                   &                        &              & -0.0002***             & -0.0002***             & 5.664e-05***   & 5.614e-05***   \\
                      &                        &              & (-4.8043)              & (-4.5439)              & (3.1030)       & (3.0350)       \\
acceleration          &                        &              & -0.5780***             & -0.5815***             & 0.1629***      & 0.1637***      \\
                      &                        &              & (-12.196)              & (-11.837)              & (10.515)       & (10.247)       \\
Intercept & -1.0327***             & 0.6202***    & 0.9134***              & 0.5667***              & 0.1704***      & 0.2480***      \\
                      & (-12.484)              & (19.571)     & (8.4296)               & (4.1454)               & (3.9879)       & (5.0004)       \\
  &  &  &  &  &  &  \\
Observations & 992 & 992 & 992 & 992 & 992 & 992 \\
R-squared             & 0.0317 & 0.0132 & 0.3743 & 0.3879 & 0.2170 & 0.2226 \\
\end{tabular}


==> TAB/reg_sophi_description.tex <==
\begin{tabular}{lcccc}
 & (1) & (2) & (3) & (4) \\
Dep. Variable           & Absolute Profits     & Percentage Profits     & Volume (ETH)     & Holding Period (hours)     \\
  &  &  &  &  \\
Sophisticated & 0.0214***            & 15.945***              & -0.0272***       & -1.1330***                 \\
                        & (7.8519)             & (4.7400)               & (-8.4040)        & (-13.558)                  \\
Intercept & 0.1131***            &                        &                  &                            \\
                        & (144.11)             &                        &                  &                            \\
  &  &  &  &  \\
Observations & 738,419 & 738,419 & 738,419 & 738,419 \\
R-squared               & 0.2977 & 0.2267 & 0.6521 & 0.1269 \\
Time FEs &  &  &  &  \\
Event FEs & Yes & Yes & Yes & Yes \\
\end{tabular}


==> TAB/reg_sophi_description_2.tex <==
\begin{tabular}{lcccccccccc}
 & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) \\
Dep. Variable         & Percentage Profits   & Volume (ETH)   & Holding Period (hours)   & Trades      & Transactions & Total Value & Inception & DEX Liquidity & liquid      & Sophisticated \\
  &  &  &  &  &  &  &  &  &  &  \\
Sophisticated & 22.177***            & 6.6398***      & 1.8220***                & 18.693***   & 715.74***      & 274.28***   & -15.478***     & 35.819***   & 1.4487***   & 1.0000***       \\
                      & (34.028)             & (91.268)       & (49.537)                 & (130.90)    & (106.01)       & (24.137)    & (-8.1788)      & (28.347)    & (17.034)    & (3.967e+16)     \\
Intercept & 72.745***            & 1.8545***      & 5.9422***                & 3.7157***   & 372.74***      & 273.25***   & 1.876e+04***   & 36.405***   & 1.8551***   & -1.274e-15***   \\
                      & (169.20)             & (125.18)       & (252.68)                 & (208.54)    & (218.53)       & (60.970)    & (2.111e+04)    & (89.628)    & (62.793)    & (-352.29)       \\
  &  &  &  &  &  &  &  &  &  &  \\
Observations & 159,037 & 159,037 & 159,037 & 159,037 & 159,037 & 159,037 & 159,037 & 159,037 & 159,037 & 159,037 \\
R-squared             & 0.0043 & 0.1116 & 0.0094 & 0.2448 & 0.1260 & 0.0046 & 0.0004 & 0.0081 & 0.0027 & 1.0000 \\
\end{tabular}


==> TAB/sophi_agents.tex <==
\begin{tabular}{lrrrrrr}
 & Count & Mean & Std & 10\% & 50\% & 90\% \\
Absolute Profits & 144,121 & 0.39 & 1.89 & -0.12 & 0.10 & 1.00 \\
Percentage Profits & 144,121 & 81.07 & 174.20 & -22.25 & 34.77 & 206.25 \\
Volume (ETH) & 144,121 & 1.00 & 2.53 & 0.10 & 0.38 & 2.00 \\
Volume (USD) & 144,121 & 2,184.85 & 5,646.06 & 193.38 & 784.60 & 4,423.79 \\
Holding Period (hours) & 144,121 & 4.56 & 7.44 & 0.00 & 0.80 & 15.82 \\
Trades & 144,121 & 2.37 & 3.50 & 1.00 & 1.00 & 4.00 \\
\end{tabular}


==> TAB/sophi_agents_2.tex <==
\begin{tabular}{lrrrrrr}
 & Count & Mean & Std & 10\% & 50\% & 90\% \\
Absolute Profits & 35,453 & 3.66 & 8.41 & 0.20 & 1.50 & 8.17 \\
Percentage Profits & 35,453 & 95.01 & 91.55 & 24.61 & 70.22 & 189.00 \\
Volume (ETH) & 35,453 & 8.45 & 13.29 & 1.18 & 3.99 & 19.22 \\
Volume (USD) & 35,453 & 18,776.99 & 29,943.63 & 2,459.16 & 8,682.58 & 43,264.85 \\
Holding Period (hours) & 35,453 & 7.76 & 5.28 & 1.86 & 6.90 & 14.60 \\
Trades & 35,453 & 22.35 & 26.47 & 6.00 & 13.00 & 47.00 \\
\end{tabular}


==> TAB/summary_panel.tex <==
\begin{tabular}{lrrrrrr}
 & count & mean & std & 10\% & 50\% & 90\% \\
Price & 3,511,676 & 0.92 & 2.19 & 0.04 & 0.22 & 2.01 \\
Floor & 3,534,040 & 0.80 & 2.05 & 0.03 & 0.18 & 1.73 \\
Return & 3,508,406 & 5.63 & 44.04 & -16.46 & 0.00 & 19.62 \\
Volume & 3,535,662 & 1.24 & 4.42 & 0.00 & 0.00 & 2.38 \\
Sales & 3,535,662 & 1.66 & 4.42 & 0.00 & 0.00 & 4.00 \\
Minted & 3,535,662 & 8,102.61 & 7,998.05 & 623.00 & 7,795.00 & 11,312.00 \\
Supply & 3,440,668 & 6,467.23 & 9,027.44 & 341.00 & 3,974.00 & 11,111.00 \\
Turnover & 3,439,122 & 0.33 & 1.34 & 0.00 & 0.02 & 0.46 \\
Capitalization & 3,534,040 & 5,254.65 & 15,264.94 & 70.83 & 1,100.31 & 9,745.52 \\
Age & 3,535,662 & 2,739.42 & 2,095.13 & 443.00 & 2,307.00 & 5,648.00 \\
\end{tabular}

